Shai: Enforcing Data-Specific Policies with Near-Zero Runtime Overhead

Data retrieval systems such as online search engines and online social networks must comply with the privacy policies of personal and selectively shared data items, regulatory policies regarding data retention and censorship, and the provider's own policies regarding data use. Enforcing these policies is difficult and error-prone. Systematic techniques to enforce policies are either limited to type-based policies that apply uniformly to all data of the same type, or incur significant runtime overhead. This paper presents Shai, the first system that systematically enforces data-specific policies with near-zero overhead in the common case. Shai's key idea is to push as many policy checks as possible to an offline, ahead-of-time analysis phase, often relying on predicted values of runtime parameters such as the state of access control lists or connected users' attributes. Runtime interception is used sparingly, only to verify these predictions and to make any remaining policy checks. Our prototype implementation relies on efficient, modern OS primitives for sandboxing and isolation. We present the design of Shai and quantify its overheads on an experimental data indexing and search pipeline based on the popular search engine Apache Lucene.

==> background.tex <==
\section{Background}
\label{sec:background}

\subsection{Capsicum}
Capsicum~\cite{capsicum} provides capability primitives for UNIX 
operating systems. These primitives provide an OS-supported sandboxing 
mechanism. Capsicum introduces two core primitives: 
\textit{capabilities} and \textit{capability mode}. A capability is a 
file descriptor with an associated access right (e.g., read-only, or 
read-write). Capability mode ensures process isolation. A process in 
capability mode can access only process-local information (e.g., open 
file descriptors), while accesses to global namespaces (e.g., file 
system's and processes' namespaces) and several management interfaces 
(such as devices, and kernel modules) are denied.
%Denying access to global namespaces is critical to isolate a process, 
%otherwise it could learn information about the system by querying 
%those 
%global namespaces (e.g., does a particular file system path exist?).
A process in capability mode cannot create capabilities outside its 
current capability set (since creating such capabilities requires 
access to global namespaces).
%Capability mode denies access to global 
%namespaces (e.g., filesystem and processes) and several management 
%interfaces (such as devices, and kernel modules) to maintain process 
%isolation. Thus, a process in capability mode cannot, on its own, name 
%system's resources (and therefore cannot create further capabilities) 
%outside its current capability set.
Typically, a program uses these primitives to limit its capabilities 
(following the principle of least privilege), then enters capability 
mode. Henceforth, damages by a compromise are limited to what is 
accessible under its capabilities.

\sysB\ uses Capsicum for process sandboxing and capabilities to ensure 
that applications can perform only select flows (whose compliance is 
established statically), and therefore avoiding the overhead of I/O 
interception for such flows.
% (in contrast to relying on I/O 
%interception to track data flows and enforce policies in \sysA).

\subsection{Light-weight contexts}
Light-weight contexts (\textit{lwCs}~\cite{lwc}) are an OS abstraction 
which provides independent units of protection, privilege, and 
execution \textit{within a process}. A process may contain multiple 
\textit{lwCs}, each with their own (or selectively shared) virtual 
memory mappings, file descriptor table, and credentials/capabilities. 
\textit{lwCs} are orthogonal to execution threads; a thread can switch 
between \textit{lwCs} through system calls. A \textit{lwC} switch is 
efficient as it avoids scheduling overhead (compared to the context 
switch of a process/thread). The \textit{lwC} API enables efficient 
compartmentalization and monitoring, all of which are crucial to \sysB\ 
as we detail next.

\sysB\ relies on \textit{lwCs} (coupled with Capsicum) for its runtime 
architecture. In \sysB, each process has a privileged monitor 
\textit{lwC} and possibly many Capsicum-sandboxed (unprivileged) 
application \textit{lwCs}. The monitor \textit{lwC} runs the reference 
monitor which creates capabilities after validating that the compliance 
conditions. Each application \textit{lwC} maps to one client and can 
acquire capabilities (from the monitor \textit{lwC}) to perform 
compliant accesses. Switching between \textit{lwCs} is efficient and 
incurs little overhead when invoking the monitor \textit{lwC} to 
acquire capabilities. The monitor \textit{lwC} protects the integrity 
of the reference monitor (by isolating it from application 
\textit{lwCs}), and the application \textit{lwCs} prevent accidental 
leakage of private information across user sessions (by isolating them 
from one another). The application \textit{lwC}'s system calls which 
require capabilities outside its current capability set are 
redirected by the underlying OS to the monitor \textit{lwC}. \sysB\ 
relies on this redirection to intercept I/O to data items outside the 
capability set of application \textit{lwCs}.

\if 0
In \sysB, each client session is mapped to a \textit{lwC}, which has 
capabilities on the compliant flows permitted for that client. This 
enables a single process to safely serve multiple clients concurrently. 
Additionally, \sysB\ relies on the \textit{lwC} monitoring facility 
(coupled with Capsicum) to efficiently grant capabilities as needed 
after satisfying the associated runtime checks. Here, a client 
\textit{lwC} runs in capability mode, whereas the privileged monitor 
\textit{lwC} runs in normal mode (thus, can create capabilities as 
needed). The client \textit{lwC} system calls which require 
capabilities outside the client \textit{lwC}'s capability set are 
redirected by the underlying OS to the monitor \textit{lwC}, which in 
turn, can decide to either grant the needed capability or not.
\fi
